Using Predicted Weights for Ad Delivery

We study the performance of a proportional weights algorithm for online capacitated bipartite matching modeling the delivery of impression ads. The algorithm uses predictions on the advertiser nodes to match arriving impression nodes fractionally in proportion to the weights of its neighbors. This paper gives a thorough empirical study of the performance of the algorithm on a data-set of ad impressions from Yahoo! and shows its superior performance compared to natural baselines such as a greedy water-filling algorithm and the ranking algorithm. The proportional weights algorithm has recently received interest in the theoretical literature where it was shown to have strong guarantees beyond the worst-case model of algorithms augmented with predictions. We extend these results to the case where the advertisers' capacities are no longer stationary over time. Additionally, we show the algorithm has near optimal performance in the random-order arrival model when the number of impressions and the optimal matching are sufficiently large.

==> algo.tex <==
\section{Proportional Weights in the i.i.d. Setting}\label{sec:algo}

Use $A$ and $I$ to represent the set of advertisers and impressions respectively. Define $n:=|A|$ and $m:=|I|$.
	For a set of proportional weights $\alpha$ and a impression subset $S\subseteq I$, let $Alloc_a(\alpha,S)$ be the allocation of advertiser $a$ using weights $\alpha$ if given impression set $S$. Furthermore, define \[R_a(\alpha,S) := \min\{Alloc_a(\alpha,S),\frac{|S|}{m}C_a  \}\] and \[R(\alpha,S) :=\sum_{a\in A}R_a(\alpha,S).\] 
	For simplicity, when $S=I$, we drop $S$ from the arguments.
	
	%Let $n$ and $m$ be the number of advertisers and impressions respectively.
	
	
	\begin{theorem}\label{thm:iid_weight}
		Assume that each impression is i.i.d. sampled from an unknown distribution. 
		For any $\sigma,\epsilon,\delta \in (0,1)$, when $m=O(\frac{n^2}{\sigma\epsilon^4}\ln(\frac{n}{\delta}))$, if a set of weights $\alpha$ has \[R(\alpha,S) \geq (1-\epsilon)\opt(S)>(1-\epsilon)\epsilon \sigma m,\]
		where $S$ is the set of first $\sigma m$ impressions, with probability at least $1-O(\delta)$, we have
		\[ R(\alpha) \geq (1-O(\epsilon))\opt. \]
	\end{theorem}

	\begin{proof}
		The basic framework of this proof is first proving 
		\begin{equation}\label{eq:iid_1}
			R(\alpha) \approx \frac{1}{\sigma}R(\alpha,S), 
		\end{equation}
		and then showing 
		\begin{equation}\label{eq:iid_2}
			\frac{1}{\sigma}\opt(S) \approx \opt. 
		\end{equation}
		Finally, according to the if condition in Theorem~\ref{thm:iid_weight}, this proof can be completed.
		
		Since $R_a(\alpha,S) := \min\{Alloc_a(\alpha,S),\sigma C_a\} $, once $Alloc_a(\alpha,S) \approx \sigma Alloc_a(\alpha) $ holds for each advertiser $a$, Eq.~\eqref{eq:iid_1} is proved.
		Let $x_{i,a}(\alpha)$ be the proportion of impression $i$ assigned to advertiser $a$ when using weights $\alpha$. Clearly,
		\[ Alloc_a(\alpha,S) = \sum_{i\in S} x_{i,a}(\alpha). \]
		
		Noting that each impression is i.i.d. sampled, we have
		\[ \E(Alloc_a(\alpha,S)) = \sigma m \E(x_{i,a} (\alpha) )=\sigma \E(Alloc_a(\alpha)), \]
		indicating that the only thing needed to prove is \[ Alloc_a(\alpha,S) \approx \E(Alloc_a(\alpha,S)).  \] In the following, we prove the above equation does not hold with probability at most $O(\delta/(n(\log n)^n))$. Then due to the union bound of total $n$ advertisers and $O((\log n)^n)$ possible sets of proportional weights, the above equation holds for any advertiser and any set of weights with probability at least $1-O(\delta)$.
		
		For simplicity, use $X$ and $\mu$, respectively, to denote $Alloc_a(\alpha,S)$ and $\E(Alloc_a(\alpha,S) )$. Employing Chernoff bound, 
		\begin{equation}\label{eq:chernoff}
			\begin{aligned}
			&\Pr[ |X -\mu |\geq \epsilon^2 \mu+ \frac{\epsilon^2\sigma m}{n} ] \\
			& \leq 2\exp(-\frac{1}{3}\mu \epsilon^4(1+\frac{\sigma m}{n\mu})^2) \\
			& = 2\exp (-\frac{1}{3} \epsilon^4(\mu + \frac{\sigma^2m^2}{n^2\mu} + \frac{2\sigma m}{n}))\\
			& \leq 2\exp(-\frac{ 4\sigma m \epsilon^4}{3n}).
			\end{aligned}
		\end{equation}		
		
		The absolute loss $\frac{\epsilon^2\sigma m}{n} $ can be tolerated because we assume that $\opt(S) \geq \epsilon \sigma m$ in the theorem. Summing over all advertisers, we loss at most $\epsilon \opt(S)$. When $m=O(\frac{n^2}{\sigma\epsilon^4}\ln(\frac{n}{\delta}))$, we have
		\begin{equation*}
		    \begin{aligned}
		      \Pr[ |X -\mu |\geq \epsilon^2 \mu+ \frac{\epsilon^2\sigma m}{n} ] &\leq 2\exp(-\frac{ 4\sigma m \epsilon^4}{3n})\\
		      &= O(\frac{\delta}{ n(\log n)^n}),      
		    \end{aligned}
		\end{equation*}
		
		completing the proof of Eq.~\eqref{eq:iid_1}.
		
		To show that Eq.~\eqref{eq:iid_2} holds, we need to recall the proof of the near-optimality of the proportional weights $\alpha$. In that proof, the approximation ratio is proved by partitioning $A$ into two sets $A_0, A_1$, and constructing a cut whose value is $|N(A_0)|+C(A_1)$, where $N(A_0)$ is the set of impressions adjacent to any $a\in A_0$ and $C(A_1)=\sum_{a\in A_1}C_a$. Then, that proof shows
		\[ R(\alpha) \geq (1-\epsilon)  (|N(A_0)|+C(A_1) )\geq (1-\epsilon) \opt. \]
		Clearly, due to $\opt \geq R(\alpha)$, we know 
		$|N(A_0)|+C(A_1)\approx \opt.$
		
		Now restricted on the first $\sigma m$ impressions, we have
		\[ |N(A_0) \cap S | + \sigma C(A_1) \approx \opt(S). \]
		 Thus, once we show that $|N(A_0) \cap S |  \approx \sigma |N(A_0)|$ with high probability, 
		 \begin{equation*}
		     \begin{aligned}
		       \opt(S) &\approx |N(A_0) \cap S | + \sigma C(A_1)  \\
		       &\approx \sigma (|N(A_0)|+C(A_1)  ) \\
		       &\geq \sigma \opt,
		     \end{aligned}
		 \end{equation*}
		 completing the proof of Eq.~\eqref{eq:iid_2}.
		 
		 Let $y_i$ be an indicator of impression $i$. If $i \in N(A_0)$, $y_i=1$. Otherwise, $y_i = 0$.
		 Clearly, $|N(A_0)\cap S| = \sum_{i\in S} y_i.$ Similar with the proof of Eq.~\eqref{eq:iid_1}, the only thing needed is showing $|N(A_0)\cap S| \approx \E(|N(A_0)\cap S| )$. Employing Chernoff bound again and following the similar algebra can finish this proof. The only difference is that we have to obtain an union bound over all $2^n$ possible cuts.
	\end{proof}
	
\subsection{Random Order}

Notice that we can obtain a similar theorem under the random order setting. Instead of using Chernoff bound, we employ a version of Bernstein’s inequality.

\begin{theorem}[Corollary 2.4 in \cite{DBLP:journals/mor/GuptaM16}]\label{thm:Bernstein}
    Let $Y=\{Y_1,...,Y_n\}$ be a set of real numbers in the interval $[0,1]$. Let $S$ be a random subset of $Y$ of size $s$ and let $Y_S=\sum_{i\in S}Y_i$. Setting $\mu=\frac{1}{n}\sum_i Y_i,$ we have that for every $\tau>0$,
    \[\Pr[|Y_S-s\mu|\geq \tau] \leq 2\exp(-\min\{ \frac{\tau^2}{8s\mu},\frac{\tau}{2}\} ). \] 
\end{theorem}

With Theorem~\ref{thm:Bernstein}, in the random order setting, we can obtain the inequality similar to Eq.~\eqref{eq:chernoff}.

\begin{equation}\label{eq:Bernstein}
    \begin{aligned}
    &\Pr[ |X -\mu |\geq \epsilon^2 \mu+ \frac{\epsilon^2\sigma m}{n} ] \\
    &\leq 2\exp(-\min \{\frac{(\epsilon^2 \mu+ \frac{\epsilon^2\sigma m}{n})^2}{8\mu},\frac{\epsilon^2 \mu+ \frac{\epsilon^2\sigma m}{n}}{2} \} )\\
    & \leq 2\exp( -\min \{ \frac{\epsilon^4\sigma m}{2n},\frac{\epsilon^2\sigma m}{2n} \} ) \\
    &\leq 2\exp ( -\frac{\sigma m\epsilon^4}{2n} ).
    \end{aligned}
\end{equation}

Since the bounds in Eq.~\eqref{eq:chernoff} and Eq.~\eqref{eq:Bernstein} are in the same magnitude, the following theorem is obtained easily.

	\begin{theorem}\label{thm:random_order}
		Assume that impressions arrive in random order. 
		For any $\sigma,\epsilon,\delta \in (0,1)$, when $m=O(\frac{n^2}{\sigma\epsilon^4}\ln(\frac{n}{\delta}))$, if a set of weights $\alpha$ has \[R(\alpha,S) \geq (1-\epsilon)\opt(S)>(1-\epsilon)\epsilon \sigma m,\]
		where $S$ is the set of first $\sigma m$ impressions, with probability at least $1-O(\delta)$, we have
		\[ R(\alpha) \geq (1-O(\epsilon))\opt. \]
	\end{theorem}




==> draft.tex <==

\newpage
\section{Exhibits}



\begin{enumerate}
    \item Robustness of IPW to neighborhood choice for impressions: [Random subset neighborhood model] Relative performance of IPW etc. against a different assignment of capacities to advertisers - for a single day only.
    
    
    


    
    \item Across-day utility of IPW: [Min-degree neighbor model] Use charts we currently have for the persistence of neighborhoods of advertisers, enforced via using smallest degree neighbors to split the impression supply equally. 
    
   
    
    
    \item Sensitivity of IPW to type variation: Keep the advertiser capacity fixed as on first day and vary the type distributions across days synthetically and plot $l_1$ difference with competitive ratio.
    Show graph of the $l_1$ difference between the impression type distributions across experiments. Show a graph plotting relation between difference in type distributions across days and competitive ratio of our PW algorithms.
    

    
 
    
    \item Arrival order variation: 5 types of orders, take the min as the measure of performance and compare - do this on the random neighborhood model. Also try across-day arrival order in this part.
    

    
    \item  Original capacity model: Show results for the worst performance across orders. Note major disparity after day 31.
    
    
    
    
\end{enumerate}


\subsection{Algorithm Description and Graph construction}

Graph: 
Each impression $v$ is denoted by a set of key-phrases $p_v$.
Count the occurrence number of each key-phrases and pick the Top-20 phrases as a base set $B$. 
Let each subset $S$ of this base set as an impression type and define the impression set $I$ in the graph to be the set of all impression types, i.e., $I:=2^B$.
Say the type of an impression $v$ is $S$ if $p_v\cap B = S$. Then, we can obtain the capacity of each impression type node.
The advertiser set $A$ is formed directly by the advertisers in the original data. Once there is a pair $(a,i)$ in the table, we connect impression type $i$ to advertisers $a$. Moreover, the edge between $a$ and any subset type of $i$ is added. We have several ways to give the advertisers capacities, in order to make sure that a perfect matching exists. For example, for each impression, send its flow randomly to its neighbours and finally, the capacity of an advertisers is the amount of flow it gets.



PW: For each impression, assign it proportionally to its neighbourhood.

IPW: For each impression, assign it proportionally to its unfull neighbourhood.
